Thermonuclear explosions as Type II supernovae

We consider a binary stellar system, in which a low-mass, of 0.6 Msun, carbon-oxygen white dwarf (WD) mergers with a degenerate helium core of 0.4 Msun of a red giant. We analyse the outcome of a merger within a common envelope (CE). We predict the observational properties of the resulting transient. We find that the double detonation of the WD, being a pure thermonuclear explosion and embedded into the hydrogen-rich CE, has a light curve with the distinct plateau shape, i.e. looks like a supernova (SN) Type IIP, with a duration of about 40 days. We find five observed SNe IIP: SN 2004dy, SN 2005af, SN 2005hd, SN 2007aa, and SN 2008bu, that match the V-band light curve of our models. Hence, we show that a thermonuclear explosion within a CE might be mistakenly identified as a SN IIP, which are believed to be an outcome of a core-collapse neutrino-driven explosion of a massive star. We discuss a number of diagnostics, that may help to distinguish this kind of a thermonuclear explosion from a core-collapse SN.

==> abstract.tex <==
%!TEX root=merger.tex

\begin{abstract}

In the present paper, we consider a binary stellar system, in which a low-mass, of 0.6~\Msun{}, carbon-oxygen white dwarf (WD) mergers with a helium core of 0.4~\Msun{} of a red giant. We analyse the outcome of the merger happening within a common-envelope, which in fact an atmosphere of a giant star. We predict the observational properties of the resulting transient. We find that the double detonation of the WD, being a pure thermonuclear explosion and being embedded into the hydrogen-rich CE, has a light curve with the distinct plateau shape, i.e. look like a supernova (SN) Type\,IIP, however, with duration of about 40~days. We found five observed SNe~IIP: SN~2004dy, SN~2005af, SN~2005hd, SN~2007aa, and SN~2008bu. Hence, we show that a thermonuclear explosion within a CE might be mistakenly identified as a SN~IIP, which are believed to be an outcome of a core-collapse neutrino-driven explosion of a massive star. We offer a few diagnostics, which can help to distinguish this kind of a thermonuclear explosion from a core-collapse SNe.
\end{abstract}

